Public Key Encryption with Secure Key Leasing

We introduce the notion of public key encryption with secure key leasing (PKE-SKL). Our notion supports the leasing of decryption keys so that a leased key achieves the decryption functionality but comes with the guarantee that if the quantum decryption key returned by a user passes a validity test, then the user has lost the ability to decrypt. Our notion is similar in spirit to the notion of secure software leasing (SSL) introduced by Ananth and La Placa (Eurocrypt 2021) but captures significantly more general adversarial strategies. In more detail, our adversary is not restricted to use an honest evaluation algorithm to run pirated software. Our results can be summarized as follows: 1. Definitions: We introduce the definition of PKE with secure key leasing and formalize security notions. 2. Constructing PKE with Secure Key Leasing: We provide a construction of PKE-SKL by leveraging a PKE scheme that satisfies a new security notion that we call consistent or inconsistent security against key leasing attacks (CoIC-KLA security). We then construct a CoIC-KLA secure PKE scheme using 1-key Ciphertext-Policy Functional Encryption (CPFE) that in turn can be based on any IND-CPA secure PKE scheme. 3. Identity Based Encryption, Attribute Based Encryption and Functional Encryption with Secure Key Leasing: We provide definitions of secure key leasing in the context of advanced encryption schemes such as identity based encryption (IBE), attribute-based encryption (ABE) and functional encryption (FE). Then we provide constructions by combining the above PKE-SKL with standard IBE, ABE and FE schemes.

==> preamble_newtheorem.tex <==
\newtheorem{theorem}{Theorem} 
\newtheorem{lemma}{Lemma} 
\newtheorem{claim}{Claim}  
\newtheorem{proposition}{Proposition} 
\newtheorem{definition}{Definition}  
\newtheorem{fact}{Fact}  
\newtheorem{remark}{Remark}  
%\newtheorem{proof}{Proof}  % Already defined by ``amsthm" package. Only include it when ``amsthm" is not used.
\newtheorem{corollary}{Corollary} 

==> preamble_usepackages_ex.tex <==

\usepackage[%
%  dvipdfmx, 
  colorlinks=true,
  citecolor=darkgreen,
  linkcolor=darkblue,
  urlcolor=darkblue,
  pagebackref=true
]{hyperref}

\usepackage{amsmath, amsfonts, amssymb, mathtools,amscd}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}

\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

\usepackage{etex}

\usepackage{arydshln} % In order to use \hdashline
\usepackage{url}
\usepackage{ifthen}
\usepackage{bm}
\usepackage{multirow}
\usepackage[dvips]{graphicx}
\usepackage[usenames]{color}
\usepackage{xcolor,colortbl} % Leave out in case the usepackage cannot be found. Not critical
\usepackage{threeparttable}
\usepackage{comment}
\usepackage{paralist,verbatim}
\usepackage{cases}
\usepackage{booktabs}
\usepackage{braket}
\usepackage{cancel} 
\usepackage{ascmac} 
\usepackage{framed}
% \usepackage{authblk}
\usepackage{pifont}
\usepackage{physics}
%\usepackage[dvipsnames]{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.6}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{maroon}{rgb}{0.5,0.1,0.1}
\definecolor{dpurple}{rgb}{0.2,0,0.65}
\definecolor{chocolate}{rgb}{0.8,0.4,0.1}

\usepackage[capitalise,noabbrev]{cleveref}
\usepackage[absolute]{textpos}
\usepackage[final]{microtype}
\usepackage[absolute]{textpos}
\usepackage{everypage}
\usepackage{autonum}

\usepackage{dsfont}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\ifnum\submission=1
\renewcommand*{\backref}[1]{}
\def\notxfont{1}
\pagestyle{plain}
\else
\fi


\ifnum\llncs=1
\renewcommand{\subparagraph}{\paragraph}
\else
\ifnum\notxfont=1
\else
\usepackage{mathpazo}
\usepackage{newtxtext}
\usepackage{helvet}
\fi
\fi


\newcommand{\heading}[1]{{\vspace{1ex}\noindent\sc{#1}}}

%%%%%%%%%%%%%%% Proof environment in non-LNCS style %%%%%%%%%%%%%%%%%%%
\newtheoremstyle{thicktheorem}%
{\topsep}
{\topsep}
{\itshape}{}%
{\bfseries}%
{.}
{ }%
{\thmname{#1}\thmnumber{ #2}%
		\thmnote{ (#3)}%
}

\newtheoremstyle{remark}%name
{\topsep}
{\topsep}
	{}%body font
	{}%indent amount
	{}%theorem head font
	{.}%punctuation after theorem head
	{ }%space after theorem head
	{\textit{\thmname{#1}}\thmnumber{ #2}%theorem head specs
			\thmnote{ (#3)}%
	}

\ifnum\llncs=0
	\theoremstyle{thicktheorem}
	\newtheorem{theorem}{Theorem}[section]
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{proposition}[theorem]{Proposition}
	\newtheorem{definition}[theorem]{Definition}

	\theoremstyle{remark}
	\newtheorem{claim}[theorem]{Claim}
	\newtheorem{remark}[theorem]{Remark}
	\newtheorem{example}[theorem]{Example}
	\newtheorem{note}[theorem]{Note}
	\newtheorem{conjecture}[theorem]{Conjecture}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


	\crefname{theorem}{Theorem}{Theorems}
	\crefname{assumption}{Assumption}{Assumptions}
	\crefname{construction}{Construction}{Constructions}
	\crefname{corollary}{Corollary}{Corollaries}
	\crefname{conjecture}{Conjecture}{Conjectures}
	\crefname{definition}{Definition}{Definitions}
	\crefname{exmaple}{Example}{Examples}
	\crefname{experiment}{Experiment}{Experiments}
	\crefname{counterexample}{Counterexample}{Counterexamples}
	\crefname{lemma}{Lemma}{Lemmata}
	\crefname{observation}{Observation}{Observations}
	\crefname{proposition}{Proposition}{Propositions}
	\crefname{remark}{Remark}{Remarks}
	\crefname{claim}{Claim}{Claims}
	\crefname{fact}{Fact}{Facts}
	\crefname{note}{Note}{Notes}

\ifnum\llncs=1
 \crefname{appendix}{App.}{Appendices}
 \crefname{section}{Sec.}{Sections}
\else
\fi

\ifnum\llncs=1
%\thispagestyle{empty}
\pagestyle{plain}
\renewcommand*{\backref}[1]{}
\else
	\renewcommand*{\backref}[1]{(Cited on page~#1.)}
	\ifnum\notxfont=1
	\else
		\usepackage{newtxtext}
	\fi
\fi


==> q-aux-secure-PKE.tex <==
% !TEX root = main.tex

\section{Quantum Auxiliary-Input Secure Public Key Encryption}
\takashi{Note that quantum auxiliary-input secure PKE will not be used in the new version. This section can be removed. Though this is not needed for the current work, we may also work on quantum auxiliary-input secure PKE as another project since this may be of independent interest.} 
\subsection{Definition}
We define CPA security w.r.t. quantum auxiliary inputs as a quantum analog of the definition given in \cite{TCC:DGKPV10}. 

\begin{definition}[CPA Security w.r.t. Quantum Auxiliary Inputs]\label{def:q-aux-secure_PKE}
Let $\PKE$ be a PKE scheme with the message space $\Xs$. 
Let $\Sset$ be a set of QPT algorithms $\qS$ that takes a key pair $(\ek,\dk)$ of $\PKE$ and outputs a quantum state. 
We say that $\PKE$ is CPA secure w.r.t. 
quantum auxiliary inputs from $\Sset$ if it satisfies the following requirement, formalized from the experiment $\expb{\PKE,\qA,\qS}{ai}{cpa}(1^\secp,\coin)$ between an adversary $\qA$ and a challenger w.r.t. an auxiliary input sampler $\qS\in \Sset$:
        \begin{enumerate}
            \item  The challenger runs $(\ek,\dk)\gets\KG(1^\secp)$ 
            and 
            $\qaux\leftarrow \qS(\ek,\dk)$ 
            and sends $\ek$ and $\qaux$ to $\qA$.
            \item $\qA$ sends $(\msg_0^*,\msg_1^*)\in \Xs^2$ 
            to the challenger. 
            \item The challenger generates $\ct^*\la\Enc(\ek,\msg_\coin^*)$ and sends $\ct^*$ to $\qA$.
            \item $\qA$ outputs a guess $\coin^\prime$ for $\coin$. The challenger outputs $\coin'$ as the final output of the experiment.
        \end{enumerate}
        For any QPT $\qA$ and $\qS\in \Sset$, it holds that
\begin{align}
\advb{\PKE,\qA,\qS}{ai}{cpa}(\secp) \seteq \abs{\Pr[\expb{\PKE,\qA,\qS}{ai}{cpa} (1^\secp,0) \ra 1] - \Pr[\expb{\PKE,\qA,\qS}{ai}{cpa} (1^\secp,1) \ra 1] }\leq \negl(\secp).
\end{align}
\end{definition}

Following \cite{TCC:DGKPV10}, we define the following special cases of the class of quantum auxiliary inputs. 
The first is bounded-length quantum auxiliary inputs.
\begin{definition}[QLB-CPA Security]\label{def:QLB-C
PA}
For a function $\ell:\mathbb{N}\rightarrow \mathbb{N}$, let $\Sset_\bdd(\ell(\secp))$ be the set of all QPT algorithms $\qS$ whose output length is at most $\ell(\secp)$-qubit on input $(\ek,\dk)\leftarrow \KG(1^\secp)$. We say that a PKE scheme $\PKE$ is $\ell(\secp)$-QLB-CPA (quantum-length-bounded CPA) secure if it is CPA secure w.r.t. quantum auxiliary inputs from $\Sset_\bdd(\ell(\secp))$. 
\end{definition}

The second is quantum auxiliary inputs from which it is hard to recover the decryption key. 
\begin{definition}[QAI-CPA Security]\label{def:QAI-C
PA}
For a function $f:\mathbb{N}\rightarrow [0,1]$, let $\Sset_\ow(f(\secp))$ be the set of all QPT algorithms $\qS$ such that for any QPT adversary $\A$, we have 
\begin{align}
    \Pr\left[\A(\qaux)\rightarrow \dk 
    \middle |
\begin{array}{ll}
(\ek,\dk)\leftarrow \KG(1^\secp)\\
\qaux \leftarrow \qS(\ek,\dk)
\end{array}
    \right]
    \le 
    f(\secp).
\end{align}
We say that a PKE scheme $\PKE$ is $f(\secp)$-QAI-CPA (quantum auxiliary input CPA) secure if it is CPA secure w.r.t. quantum auxiliary inputs from $\Sset_\ow(f(\secp))$. 
When $\PKE$ is $(1/\poly(\secp))$-QAI-CPA secure for all polynomials $\poly$, we simply say that it is QAI-CPA secure. 
\end{definition}

Finally, we define a weaker variant of the QAI-CPA security where we only consider quantum auxiliary inputs from which it is hard to recover the decryption key \emph{even if additionally given the encyption key}. 
\begin{definition}[wQAI-CPA Security]\label{def:wQAI-C
PA}
For a function $f:\mathbb{N}\rightarrow [0,1]$, let $\Sset_{\ekow}(f(\secp))$ be the set of all QPT algorithms $\qS$ such that for any QPT adversary $\A$, we have 
\begin{align}
    \Pr\left[\A(\ek,\qaux)\rightarrow \dk 
    \middle |
\begin{array}{ll}
(\ek,\dk)\leftarrow \KG(1^\secp)\\
\qaux \leftarrow \qS(\ek,\dk)
\end{array}
    \right]
    \le 
    f(\secp).
\end{align}
We say that a PKE scheme $\PKE$ is $f(\secp)$-wQAI-CPA (weak quantum auxiliary input CPA) secure if it is CPA secure w.r.t. quantum auxiliary inputs from $\Sset_{\ekow}(f(\secp))$.
When $\PKE$ is $(1/\poly(\secp))$-wQAI-CPA secure for all polynomials $\poly$, we simply say that it is wQAI-CPA secure. 
\end{definition}

We have the following relationship among the above security notions similarly to the classical case~\cite[Lemma 4]{TCC:DGKPV10}.
\begin{lemma}
Suppose that a PKE scheme $\PKE$ has public key length $t(\secp)$ and min-entropy $k(\secp)$ of secret keys. \takashi{to be defined.} Then, we have the following:
\begin{enumerate}
    \item If $\PKE$ is $f(\secp)$-QAI-CPA secure, then $\PKE$ is $f(\secp)$-wQAI-CPA secure.
     \item If $\PKE$ is $f(\secp)$-wQAI-CPA secure, then $\PKE$ is $(2^{-t(\secp)}f(\secp))$-QAI-CPA secure.
     \item If $\PKE$ is $f(\secp)$-QAI-CPA secure, then $\PKE$ is $(k(\secp)-\log(1/f(\secp)))$-QLB-CPA secure.
\end{enumerate}
\end{lemma}

\begin{remark}
For the purpose of this paper, we only need wQAI-CPA security. We also define QLB-CPA and QAI-CPA security because they may be of independent interest. We give results on QLB-CPA and QAI-CPA secure PKE schemes as corollaries of our construction of wQAI-CPA secure PKE in Appendix \takashi{to be written}. 
\end{remark}


We remark that wQAI-CPA security by itself does not ensure any meaningful security. For example, if we consider a trivial scheme where we always have $\dk=\ek$, it always satisfies wQAI-CPA security since then $\Sset_{\ekow}(f(\secp))$ is the empty set for any $f(\secp)$. Thus, when we use wQAI-CPA secure PKE schemes, we also require the following mild security notion, which requires that one cannot recover a decryption key only from an encryption key.
\begin{definition}[Unpredictable Decryption Keys]
We say that a PKE scheme $\PKE$ has unpredictable decryption keys if the support of $\KG$ is efficiently recognizable, i.e., there is a classical polynomial-time algorithm to decide if a given pair $(\ek,\dk)$ belongs to the support of $\KG(1^\secp)$, and for any QPT algorithm $\qA$, we have
\begin{align}
\Pr\left[(\ek,\widetilde{\dk})\in \KG(1^\secp) \middle | 
\begin{array}{ll}
(\ek,\dk)\leftarrow \KG(1^\secp)\\
\widetilde{\dk}\leftarrow \qA(\ek)
\end{array}
\right]\le \negl(\secp).
\end{align}
\end{definition}

By additionally assuming the unpredictable decryption key property, wQAI-CPA security ensures meaningful security. In particular, it is easy to see that if a wQAI-CPA secure PKE scheme has unpredictable decryption keys, then it is IND-CPA secure. 


\if0
\begin{definition}[wQAI-CPA Security]\label{def:w-q-aux-secure_PKE}
We say that a PKE scheme $\PKE$  with the message space $\Xs$ is weak quantum auxiliary-input-CPA (wQAI-CPA) secure if the following is satisfied.
    There exist a QPT algorithm $\qExt$ and a polynomial $\poly$ such that
    such that for any $(\ek,\dk)\leftarrow \KG(1^\secp)$, a QPT adversary $\qA$, a polynomial-size quantum state $\qadv$, $(\msg_0^*,\msg_1^*)\in \Xs^2$, and a function $\epsilon:\mathbb{N}\rightarrow [0,1]$, if we have
    \begin{align}
    \left|
    \Pr\left[
\qA(\qadv,\ct^*_0)\rightarrow 1
\ \middle |
\begin{array}{ll}
\ct^*_0\gets\Enc(\ek,\msg_0^*)
\end{array}
\right] 
-
    \Pr\left[
\qA(\qadv,\ct^*_1)\rightarrow 1
\ \middle |
\begin{array}{ll}
\ct^*_0\gets\Enc(\ek,\msg_1^*)
\end{array}
\right] 
\right|\ge \epsilon(\secp),
    \end{align}
then we have 
\begin{align}
\Pr\left[
 \qExt(\ek,\qA,\qadv,\msg_0^*,\msg_1^*)=\dk\right]\geq \poly(\epsilon(\secp)).
\end{align}
\end{definition}

\begin{remark}
By taking the contrapositive, the wQAI-CPA security defined above roughly corresponds to the quantum analog of the wAI-CPA security as defined in \cite{TCC:DGKPV10}. 
This is why we call the above definition wQAI-CPA security instead of QAI-security. 
The work \cite{TCC:DGKPV10} also define a stronger security notion called AI-CPA security which roughly means that the extractor does not need to take $\ek$ as input in the above formalization.  They show that we can reduce the AI-CPA security to the wAI-CPA security with a multiplicative security loss of factor $2^{|\ek|}$ where $|\ek|$ denotes the length of encryption keys. We can define a quantum analog, QAI-CPA security, of AI-CPA security and show a similar reduction from the QAI-CPA security to wQAI-CPA security. Since we only need wQAI-CPA security for our purpose, we omit details on QAI-CPA security.
\end{remark}
\fi

\subsection{Construction}
We give a construction of wQAI-CPA secure PKE scheme that has decryption keys based on batch encryption.
\begin{theorem}
If there is a batch encrytpion scheme, then there exists a wQAI-CPA secure PKE scheme that has decryption keys.
\end{theorem}

Our construction is identical to to the scheme by Brakerski et al.~\cite{EC:BLSV18}. They show leakage resilience of their scheme and mention that the security w.r.t. (classical) auxiliary inputs should follow in a similar manner without giving a proof. By extending their proof of leakage resilience, we show that the scheme is also secure w.r.t. quantum auxliary inputs (i.e., wQAI-CPA secure) if we assume post-quantum security for the batch encryption. The proof is similar to theirs except that we rely on Goldreich-Levin theorem with quantum auxiliary inputs~\cite{C:CLLZ21} instead of the left-over-hash lemma. 


Let $\BE=(\BE.\Setup, \BE.\KG, \BE.\Enc, \BE.\Dec)$ is an IND-CPA secure batch encryption scheme with public key length $\secp$. Then, we construct wQAI-CPA secure PKE scheme $\PKE=(\PKE.\KG,\PKE.\Enc,\PKE.\Dec)$ with one-bit message as follows where we set $n=(1+\epsilon)\secp$ for some constant $\epsilon>0$. 
We remark that we can extend it to a multi-bit message one by parallel repetition since we can show that the wQAI-CPA security and the unpredictable decryption key property are preserved under the parallel composition by a standard hybrid argument. 
\begin{description}  
\item[$\PKE.\KG(1^\secp)$:] 
On input the security parameter $1^\secp$, generate
$\crs\gets \BE.\Setup(1^\secp)$, $x\gets \bit^n$, and $h\gets \BE.\KG(\crs,x)$, and 
outputs 
an encryption key $\ek\seteq(\crs,h)$ and a decryption key $\dk\seteq x$. 

\item[$\PKE.\Enc(\ek,\msg)$:] 
On input the encryption key $\ek=(\crs,h)$ and a message $\msg\in \bit$, generate an $n$-out-of-$n$ XOR secret sharing $\{s_i\}_{i\in [n]}$ of $\msg$, i.e., uniformly choose $s_i\gets \bit$ for $i\in [n-1]$ and set $s_n\seteq \bigoplus_{i\in[n-1]}r_i\oplus \msg$ (so that we have $\bigoplus_{i\in[n]}s_i=\msg$), set $\msg_{i,0}=\msg_{i,1}=s_i$ for $i\in [n]$, generate
$\ct\gets \BE.\Enc(\crs,h,\{\msg_{i,b}\}_{i\in[n],b\in\bit})$, and output $\ct$. 

\item[$\PKE.\Dec(\dk,\ct)$:] 
On the decryption key $\dk=x$ and a ciphertext $\ct$, compute $\{\tilde{s}_i\}_{i\in[n]}\leftarrow \BE.\Dec(\crs,x,\ct)$
and outputs $\tilde{\msg}\seteq \oplus_{i\in [n]}\tilde{s}_i$.
\end{description}

The correctness of $\PKE$ easily follows from the correctness of $\BE$. 

\begin{theorem}
If $\BE$ is IND-CPA secure, then $\PKE$ is wQAI-CPA secure and has unpredictable decryption keys. 
\end{theorem}
\begin{proof}
The unpredictable decryption key property of $\PKE$ directly follows from the IND-CPA security of $\BE$ and \Cref{lem:one-way_KG}. 
% easily follows from the IND-CPA security of $\BE$ because the IND-CPA security of $\BE$ implies that $\BE.\KG(\crs,\cdot)$ is collision-resistant and sufficiently length-decreasing collision-resistant function is one-way.  

In the following, we prove wQAI-CPA security of $\PKE$. 
%Suppose that it does not hold. Then, there exists a QPT adversary $\qA$ and $\qS$ such that 
%$\advb{\PKE,\qA,\qS}{ai}{cpa}(\secp)$ as defined in \Cref{def:q-aux-secure_PKE} is non-negligible  
Let $\qS$ be a QPT algorithm that belongs to $\Sset_{\ekow}$ (as defined in \Cref{def:wQAI-C
PA}), i.e.,  
for any QPT algorithm $\qB$, we have
\begin{align} 
    \Pr\left[\qB(\crs,h,\qaux)\rightarrow x 
    \middle |
\begin{array}{ll}
\crs \leftarrow \BE.\Setup(1^\secp)\\
x \gets \bit^n\\
h \gets \BE.\KG(\crs,x)\\
\qaux \leftarrow \qS(\crs,h,x)
\end{array}
    \right]\le \negl(\secp). \label{eq:hard_to_find_x}
\end{align}

For a QPT adversary $\qA$, 
we consider the following sequence of games.
Let $\cE_{\rm xx}$ be the event that $\game{\rm xx}$ outputs $1$. 
%For $i$, let $\E_i$ denote the event that $\Game_i$ outputs $1$. 
\begin{itemize}
\item[$\game{0}$:] This is the real experiment $\expb{\PKE,\qA,\qS}{ai}{cpa} (1^\secp,0)$ as defined in \Cref{def:q-aux-secure_PKE} (with $\coin = 0$) where we assume $\msg^{(b)}=b$ without loss of generality since we consider a single-bit message scheme. That is, the game works as follows.
\begin{enumerate}
            \item  The challenger generates $\crs\gets \BE.\Setup(1^\secp)$, $x\gets \bit^n$, and $h\gets \BE.\KG(\crs,x)$, 
            sets $\ek\seteq (\crs,h)$ and $\dk\seteq x$, 
            generates 
            $\qaux\leftarrow \qS(\ek,\dk)$. 
            Then, the challenger generates an $n$-out-of-$n$ XOR secret sharing $\{s_i\}_{i\in [n]}$ of $0$,  sets $\msg_{i,0}=\msg_{i,1}=s_i$ for $i\in [n]$, generates
$\ct^*\gets \BE.\Enc(\crs,h,\{\msg_{i,b}\}_{i\in[n],b\in\bit})$,
         and sends $\ek$, $\qaux$, and $\ct^*$ to $\qA$.
            \item $\qA$ outputs a guess $\coin^\prime$ for $\coin$. The challenger outputs $\coin'$ as the final output of the game.
        \end{enumerate}
\if0
\begin{enumerate}
            \item  The challenger generates $\crs\gets \BE.\Setup(1^\secp)$, $x\gets \bit^n$, and $h\gets \BE.\KG(\crs,x)$, 
            sets $\ek\seteq (\crs,h)$ and $\dk\seteq x$, 
            generates 
            $\qaux\leftarrow \qS(\ek,\dk)$, 
            and sends $\ek$ and $\qaux$ to $\qA$. 
            \item $\qA$ sends $(\msg^{(0)},\msg^{(1)})\in \bit^{2}$ 
            to the challenger. 
            \item 
            The challenger generates an $n$-out-of-$n$ XOR secret sharing $\{s_i\}_{i\in [n]}$ of $\msg^{(0)}$,  sets $\msg_{i,0}=\msg_{i,1}=s_i$ for $i\in [n]$, generate
$\ct^*\gets \BE.\Enc(\crs,h,\{\msg_{i,b}\}_{i\in[n],b\in\bit})$
         and sends $\ct^*$ to $\qA$.
            \item $\qA$ outputs a guess $\coin^\prime$ for $\coin$. The challenger outputs $\coin'$ as the final output of the game.
        \end{enumerate}
\fi
\item[$\game{1}$:] This game is identical to the previous game except that for all $i\in[n]$, $\msg_{i,1-x_i}$ is independently and uniformly chosen instead of set to be $s_i$. We remark that we still set $\msg_{i,x_i}\seteq s_i$ for all $i\in[n]$.

By a straightforward reduction to IND-CPA security of $\BE$, we have 
\begin{align}
    |\Pr[\cE_{0}]-\Pr[\cE_{1}]|\le \negl(\secp).
\end{align}

\item[$\game{2}$:]
This game is identical to the previous game except that we modify the way of sampling $\{\msg_{i,b}\}_{i\in[n],b\in\bit}$ as follows.
The challenger randomly chooses 
$\msg_{i,0}\gets \bit$ for $i\in [n-1]$ and 
$r_i\gets \bit$ for $i\in [n]$, and sets
\begin{align}
    \msg_{n,0}^{(0)}\seteq \msg^{(0)} \oplus \left(\bigoplus_{i\in [n-1]}\msg_{i,0}\right) 
    \oplus \left(\bigoplus_{i\in [n]}x_i r_i\right)
\end{align}
and
\begin{align}
    \msg_{i,1}\seteq r_i \oplus \msg_{i,0}
\end{align}
for all $i\in [n]$.

One can see that the distribution of $\{\msg_{i,b}\}_{i\in[n],b\in\bit}$ does not change from $\game{1}$. (Think of $r_i$ as $\msg_{i,0}\oplus \msg_{i,1}$.) \takashi{more explanation needed?}
Therefore, we have 
\begin{align}
    \Pr[\cE_{1}] = \Pr[\cE_{2}].
\end{align}

\item[$\game{3}$:] 
This game is identical to the previous game except that $\{\msg_{i,b}\}_{i\in[n],b\in\bit}$ is uniformly chosen from $\bit^2n$. 


If we replace $\bigoplus_{i\in [n]}x_i r_i$ in the definition of $\msg_{n,0}^{(0)}$ in $\game{2}$ with a uniformly random bit, then the distribution of $\{\msg_{i,b}\}_{i\in[n],b\in\bit}$ becomes identical to that in $\game{3}$. 
Moreover, $x$ is used only for computing $\bigoplus_{i\in [n]}x_i r_i$ in $\game{2}$. 
Therefore, if $\qA$ distinguishes $\game{3}$ from $\game{2}$, then we can use it to construct a QPT algorithm $\qA'$ such that 
\begin{align} 
    \Pr\left[\qA'(\crs,h,\qaux,r)\rightarrow \bigoplus_{i\in [n]}x_i r_i 
    \middle |
\begin{array}{ll}
\crs \leftarrow \BE.\Setup(1^\secp)\\
x \gets \bit^n\\
h \gets \BE.\KG(\crs,x)\\
\qaux \leftarrow \qS(\crs,h,x)\\
r\gets \bit^n
\end{array}
    \right]\ge \frac{1}{2} + \epsilon(\secp).
\end{align}
for a non-negligible $\epsilon(\secp)$.
By a standard averaging argument, for at least  $(\epsilon(\secp)/2)$-fraction of $(\crs,h,\qaux)$, we have 
\begin{align} 
    \Pr\left[\qA'(\crs,h,\qaux,r)\rightarrow \bigoplus_{i\in [n]}x_i r_i 
    \middle |
\begin{array}{ll}
r\gets \bit^n
\end{array}
    \right]\ge \frac{1}{2} + \frac{\epsilon(\secp)}{2}.
\end{align}
By the quantum Goldreich-Levin theorem with quantum auxiliary inputs (\Cref{lem:QGL}), there is a QPT $\qExt$ such that for any such $(\crs,h,\qaux)$, we have  
\begin{align} 
    \Pr\left[\qExt(\qA',\crs,h,\qaux,r)\rightarrow x
    \middle |
\begin{array}{ll}
r\gets \bit^n
\end{array}
    \right]\ge \epsilon(\secp)^2.
\end{align}
Since this holds for at least $(\epsilon(\secp)/2)$-fraction of $(\crs,h,\qaux)$, we have
\begin{align} 
    \Pr\left[\qExt(\qA',\crs,h,\qaux,r)\rightarrow x
    \middle |
\begin{array}{ll}
\crs \leftarrow \BE.\Setup(1^\secp)\\
x \gets \bit^n\\
h \gets \BE.\KG(\crs,x)\\
\qaux \leftarrow \qS(\crs,h,x)\\
r\gets \bit^n
\end{array}
    \right]\ge \frac{\epsilon(\secp)^3}{2}.
\end{align}
Since we assume $\epsilon(\secp)$ is non-negligible, this contradicts \Cref{eq:hard_to_find_x}. Therefore, we have
\begin{align}
    |\Pr[\cE_{2}]-\Pr[\cE_{3}]|\le \negl(\secp).
\end{align}

%Note that $(\msg^{(0)},\msg^{(1)})$ is not used at all in $\game{3}$. Therefore, by 
By considering similar game hops to those from $\game{0}$ to $\game{3}$ in the reversed order, we can show 
\begin{align}
    |\Pr[\cE_{3}]-\Pr[\expb{\PKE,\qA,\qS}{ai}{cpa} (1^\secp,1)\ra 1]|\le \negl(\secp).
\end{align}

Combining the above, we have 
\begin{align}
    |\Pr[\expb{\PKE,\qA,\qS}{ai}{cpa} (1^\secp,0)\ra 1]-\Pr[\expb{\PKE,\qA,\qS}{ai}{cpa} (1^\secp,1)\ra 1]|\le \negl(\secp).
\end{align}
This means that $\PKE$ is wQAI-CPA secure.
\end{itemize}
\end{proof}

\noindent
\textbf{\underline{Alternative Construction.}}
We show that the dual-Regev encryption is also wQAI-CPA secure and has unpredictable encryption keys under the LWE assumption in Appendix \takashi{to be written}. Though this does not give a new feasibility result since the LWE assumption implies the existence of batch encryption, the construction is more efficient.  
